Zero-shot Unsupervised Transfer Instance Segmentation

Segmentation is a core computer vision competency, with applications spanning a broad range of scientifically and economically valuable domains. To date, however, the prohibitive cost of annotation has limited the deployment of flexible segmentation models. In this work, we propose Zero-shot Unsupervised Transfer Instance Segmentation (ZUTIS), a framework that aims to meet this challenge. The key strengths of ZUTIS are: (i) no requirement for instance-level or pixel-level annotations; (ii) an ability of zero-shot transfer, i.e., no assumption on access to a target data distribution; (iii) a unified framework for semantic and instance segmentations with solid performance on both tasks compared to state-of-the-art unsupervised methods. While comparing to previous work, we show ZUTIS achieves a gain of 2.2 mask AP on COCO-20K and 14.5 mIoU on ImageNet-S with 919 categories for instance and semantic segmentations, respectively. The code is made publicly available.

==> tables/rebuttal-stop-grad.tex <==
\setlength\tabcolsep{3.5pt}
\vspace{-4mm}
\begin{table}[!th]
\centering
\begin{tabular}{c|ccc|ccc}
          & \multicolumn{3}{c|}{\textit{\red{class-agnostic}}} & \multicolumn{3}{c}{\textit{\blue{class-aware}}} \\
stop-grad & $\maskap$ & $\maskapfifty$ & $\maskapseventyfive$ & $\maskap$ & $\maskapfifty$ & $\maskapseventyfive$\\ \hline
\xmark & 8.4 & 19.9 & 6.4 & 1.0 & 1.9 & 0.9 \\
\checkmark & 9.9 & 24.1 & 7.4 & 13.7 & 30.9 & 11.1  
\vspace{-3.5mm}
\end{tabular}
\caption{Effect of a stop-grad operation on VOC2012}
\label{tab:stop-grad}
\vspace{-5mm}
\end{table}




==> tables/rebuttal-unseen-instance-segmentation.tex <==
\vspace{-3.5mm}
\begin{table}[!th]
\centering
\begin{tabular}{l|lll}
method   & $\maskap$ & $\maskapfifty$ & $\maskapseventyfive$ \\ \hline
MaskCLIP & 0.7 & 2.0  & 0.4  \\
Ours     & 3.3 \green{($+2.6$)} & 7.2 \green{($+5.2$)} & 2.8 \green{($+2.4$)}
\vspace{-4mm}
\end{tabular}

\caption{Unsupervised instance segmentation on unseen classes}
\vspace{-7mm}
\label{tab:unseen-instance-segmentation}
\end{table}
